Discovering Strong Gravitational Lenses in the Dark Energy Survey with Interactive Machine Learning and Crowd-sourced Inspection with Space Warps

We conduct a search for strong gravitational lenses in the Dark Energy Survey (DES) Year 6 imaging data. We implement a pre-trained Vision Transformer (ViT) for our machine learning (ML) architecture and adopt Interactive Machine Learning to construct a training sample with multiple classes to address common types of false positives. Our ML model reduces 236 million DES cutout images to 22,564 targets of interest, including around 85% of previously reported galaxy-galaxy lens candidates discovered in DES. These targets were visually inspected by citizen scientists, who ruled out approximately 90% as false positives. Of the remaining 2,618 candidates, 149 were expert-classified as 'definite' lenses and 516 as 'probable' lenses, with 147 of these candidates being newly identified. Additionally, we trained a second ViT to find double-source plane lens systems, finding at least one double-source system. Our main ViT excels at identifying galaxy-galaxy lenses, consistently assigning high scores to candidates with high confidence. The top 800 ViT-scored images include around 100 of our `definite' lens candidates. This selection is an order of magnitude higher in purity than previous convolutional neural network-based lens searches and demonstrates the feasibility of applying our methodology for discovering large samples of lenses in future surveys.

==> Figures/P_Trajectory_Plots.tex <==
\begin{figure}
 \centering
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/DES_VT_3_Nov_1700_BST_trajectory_plot.pdf}
\caption{Score trajectories of a random sample of training subjects and known lens candidates. The vast majority of training subjects were correctly classified as lenses (green) or non-lenses (blue).
%High-grade known lenses are shown in green: these were present in both the training and test datasets but the scores shown here are from those placed in the test subject dataset. 
A random subset of high grade known candidates from the O'Donnell and Jacobs samples are also shown (pink), the majority of which are identified as lenses.
Subjects were originally assigned the prior probability (dashed line) and were retired (removed from the platform and not classified further) if they reached the lower probability threshold (dotted line). The histograms in the lower panel shows the final score distributions for all subjects.}
% Subsample substantially}
\label{Fig: Trajectory_Plots}
\end{figure}

